Neural Texture Puppeteer: A Framework for Neural Geometry and Texture Rendering of Articulated Shapes, Enabling Re-Identification at Interactive Speed

In this paper, we present a neural rendering pipeline for textured articulated shapes that we call Neural Texture Puppeteer. Our method separates geometry and texture encoding. The geometry pipeline learns to capture spatial relationships on the surface of the articulated shape from ground truth data that provides this geometric information. A texture auto-encoder makes use of this information to encode textured images into a global latent code. This global texture embedding can be efficiently trained separately from the geometry, and used in a downstream task to identify individuals. The neural texture rendering and the identification of individuals run at interactive speeds. To the best of our knowledge, we are the first to offer a promising alternative to CNN- or transformer-based approaches for re-identification of articulated individuals based on neural rendering. Realistic looking novel view and pose synthesis for different synthetic cow textures further demonstrate the quality of our method. Restricted by the availability of ground truth data for the articulated shape's geometry, the quality for real-world data synthesis is reduced. We further demonstrate the flexibility of our model for real-world data by applying a synthetic to real-world texture domain shift where we reconstruct the texture from a real-world 2D RGB image. Thus, our method can be applied to endangered species where data is limited. Our novel synthetic texture dataset NePuMoo is publicly available to inspire further development in the field of neural rendering-based re-identification.

==> figures/fig_pos_enc.tex <==
\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{0.49\linewidth}
        \centering
        \includegraphics[width=\textwidth]{images/pos_enc_novel_pose/gt_pos_enc_frame851_camera6.png}
        \caption{Ground Truth}
        \label{fig:pos_enc:gt}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.49\linewidth}
        \centering
        \includegraphics[width=\textwidth]{images/pos_enc_novel_pose/rec_pos_enc_frame851_camera6.png}
        \caption{Our Reconstruction}
        \label{fig:pos_enc:rec}
    \end{subfigure}
    \caption{
        %
        \textbf{Novel Pose Synthesis: NNOPCS Maps.}
        %
        We show one example from our novel~\dataabr test set for the NNOPCS maps, cf. Sec. \todo{3.1} in main paper.
        %
        %Our reconstruction reflects the overall high quality of our quantitative results in~\cref{tab:quantitative-pos-enc-depth}.
    }
    \label{fig:pos_enc}
\end{figure}

==> figures/fig_pose_enc_gt.tex <==
\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{0.49\linewidth}
        \centering
        \includegraphics[width=\textwidth]{images/color_novel_pose/pose_enc_gt_diag.png}
        % \caption{Standard Pose: Front Right}
        \label{fig:pos_enc_standard:right}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.49\linewidth}
        \centering
        \includegraphics[width=\textwidth]{images/color_novel_pose/pose_enc_gt_diag2.png}
        % \caption{Standard Pose: Front Left}
        \label{fig:pose_enc_standard:left}
    \end{subfigure}
    \caption{
        %
        \textbf{NNOPCS Maps in Neutral Pose.}
        %
        We show the neutral pose of the NNOPCS projected on two image planes, cf.~\cref{sec:positional_encoding}.
        %
        The color at each point on the mesh depends on its position in $x$-, $y$-, and $z$-direction in the neutral pose. Thus, for other poses the color at a specific position on the mesh remains the same, uniquely describing this point.}
    \label{fig:pos_enc_standard}
\end{figure}

==> figures/fig_reid_occ.tex <==
\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{\linewidth}
        \centering
        \includegraphics[width=\textwidth]{images/z_texture/z_texture_occlusions_complete_masks_kde_mask_intersection.png}
        \caption{Complete Masks}
        \label{fig:reid:occ:complete_masks}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{\linewidth}
        \centering
        \includegraphics[width=\textwidth]{images/z_texture/z_texture_occlusions_kde_mask_intersection.png}
        \caption{Occluded Masks}
        \label{fig:reid:occ:occ_masks}
    \end{subfigure}
    \caption{
        %
        \textbf{KDE of the global texture codes: Occlusions.}
        %
        The contour lines depict the KDE of the t-SNE of latent codes of our training examples.
        %
        The dots depict the position of the latent code for partially occluded examples.
        % We show the KDE of instances without (contour lines) and with (dots) occlusions.
        %
        The instances where the Holstein (texture $0$) partially occludes the Limousine (texture $11$) cow (cf.~\cref{fig:dataset_occ:image}) cluster correctly into the cluster of the Limousine cow.
        %
        See text for a discussion of the results.
        %
    }
    \label{fig:reid:occ}
\end{figure}

==> figures/fig_reid_real_world.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{images/z_texture/z_texture_real_world_combined_kde_2.png}
    \caption{
        %
        \textbf{KDE of the global texture codes: Real-World Examples.}
        %
        We show the KDE of our real-world examples (cf.~\cref{fig:real_world}).
        %
        The insets show texture $2$ and $11$.
        %
        See text for a discussion of the results.
        %
    }
    \label{fig:reid:rw}
\end{figure}
